Disentangling Trainability and Generalization in Deep Neural Networks

A longstanding goal in the theory of deep learning is to characterize the conditions under which a given neural network architecture will be trainable, and if so, how well it might generalize to unseen data. In this work, we provide such a characterization in the limit of very wide and very deep networks, for which the analysis simplifies considerably. For wide networks, the trajectory under gradient descent is governed by the Neural Tangent Kernel (NTK), and for deep networks the NTK itself maintains only weak data dependence. By analyzing the spectrum of the NTK, we formulate necessary conditions for trainability and generalization across a range of architectures, including Fully Connected Networks (FCNs) and Convolutional Neural Networks (CNNs). We identify large regions of hyperparameter space for which networks can memorize the training set but completely fail to generalize. We find that CNNs without global average pooling behave almost identically to FCNs, but that CNNs with pooling have markedly different and often better generalization performance. These theoretical results are corroborated experimentally on CIFAR10 for a variety of network architectures and we include a colab notebook that reproduces the essential results of the paper.

==> Trainability-Generalization-ICML2020 (2)/tex_zoo/body.tex <==

\section{Background}\label{sec:background}
We summarize recent developments in the study of wide random networks. We will keep our discussion relatively informal; see e.g. ~\citep{novak2018bayesian} for a more rigorous version of these arguments. To simplify this discussion and as a warm-up for the main text, we will consider the case of FCNs. Consider a fully-connected network of depth $L$ where each layer has a width $N^{(l)}$ and an activation function $\phi:\mathbb R\to\mathbb R$. In the main text we will restrict our discussion to $\phi=\text{erf}$ or $\tanh$ for clarity, however we include results for a range of architectures including $\phi= \text{ReLU}$ with and without skip connections and layer normalization in the supplementary material (see Sec.~\ref{sec:RElu-networks}). We find that the high level picture described here applies to a wide range of architectural components, though important specifics - such as the phase diagram - can vary substantially. For simplicity, we will take the width of the hidden layers to infinity sequentially: $N^{(1)} \to\infty, \dots, N^{(L-1)} \to\infty$. The network is parameterized by weights and biases that we take to be randomly initialized with $W_{ij}^{(l)}, b_i^{(l)}\sim\mathcal N(0, 1)$ along with hyperparameters, $\sigma_w$ and $\sigma_b$ that set the scale of the weights and biases respectively. Letting the $i$\textsuperscript{th} pre-activation in the $l$\textsuperscript{th} layer due to an input $x$ be given by $z^{(l)}_i(x)$, the network is then described by the recursion, for $0\leq l \leq L-1$, 
\begin{equation}\label{eq:fc_def_recap_recursion}
    z^{(l+1)}_i(x) = \frac{\sigma_w}{\sqrt {N^{(l)}}}\sum_{j=1}^{N^{(l)}}W^{(l+1)}_{ij}\phi(z^{(l)}_j(x)) + \sigma_b b^{(l+1)}_i 
\end{equation}
Notice that as $N^{(l)}\to\infty$, the sum ends up being over a large number of random variables and we can invoke the central limit theorem to conclude that the $\{z_i^{(l+1)}\}_{i\in [N^{(l+1)}]}$ are i.i.d. Gaussian with zero mean. Given a dataset of $m$ points, the distribution over pre-activations can therefore be described completely by the covariance matrix, i.e. the NNGP kernel, between neurons in different inputs $\Kl(x,x') = \mathbb E[z^{(l)}_{i}(x)z^{(l)}_{i}(x')].$ Inspecting~\eqref{eq:fc_def_recap_recursion}, we see that $\Kll$ can be computed in terms of $\Kl$ as 
\begin{align}\label{eq:fc_mft_recap_recursion-main}
    \Kll(x, x') 
    % &= \sigma_w^2\mathbb E_{(z,z')\sim\mathcal N(0,\Kl(x, x'))}[\phi(z)\phi(z')] + \sigma_b^2
    % \nonumber
     &\equiv \sigma_w^2 \mathcal T(\Kl)(x, x') + \sigma_b^2 \,
     \\
     \mathcal T(\K) & \equiv \mathbb E_{z\sim\mathcal N(0, \K)}[\phi(z)\phi(z)^T]
\end{align}
% Here $\T$ is operator from the space of positive semi-definite matrices to itself. 

\eqref{eq:fc_mft_recap_recursion-main} describes a dynamical system on positive semi-definite matrices $\mathcal K$. It was shown in~\citet{poole2016exponential} that fixed points, $\mathcal K^*(x,x')$, of these dynamics exist such that $\lim_{l\to\infty}\Kl(x,x')=\mathcal K^*(x,x')$ with $\mathcal K^*(x,x') = q^*[\delta_{x,x'} + c^*(1-\delta_{x,x'})]$ independent of the inputs $x$ and $x'$. The values of $q^*$ and $c^*$ are determined by the hyperparameters, $\sigma_w$ and $\sigma_b$. However ~\eqref{eq:fc_mft_recap_recursion-main} admits multiple fixed points (e.g. $c^* = 0, 1$) and the stability of these fixed points plays a significant role in determining the properties of the network. Generically, there are large regions of the $(\sigma_w,\sigma_b)$ plane in which the fixed-point structure is constant punctuated by curves, called phase transitions, where the structure changes; see Fig~\ref{fig:phase-diagram} for $\tanh$-networks.  

The rate at which $\mathcal K(x, x')$ approaches or departs $\mathcal K^*(x, x')$ can be determined by expanding \eqref{eq:fc_mft_recap_recursion-main} about its fixed point, $\delta\mathcal K(x, x') = \mathcal K(x, x') - \mathcal K^*(x, x')$ to find
% \footnote{More precisely, one needs to consider the Jacobian of $\T$ as an operator from positive semi-definite matrices to positive semi-definite matrices. We refer the readers to Section B of \citet{xiao18a} for more details.}
\begin{equation}
    \delta\Kll(x, x') \approx \sigma_w^2\dot{\mathcal T}(\mathcal K^*(x, x'))\delta\Kl(x, x')
\end{equation}
with $\dot{\mathcal T}(\K) = \mathbb E_{(z_1, z_2)\sim \mathcal N(0, \K)}[\dot\phi(z_1)\dot\phi(z_2)]$ and $\dot \phi$ is the derivative of $\phi$. This expansion naturally exhibits exponential convergence to - or divergence from - the fixed-point as $\delta\mathcal K^{(l)}(x, x')\sim \chi(x, x')^l$ where $\chi(x,x') = \sigma_w^2\dot{\mathcal T}(\mathcal K^*(x, x'))$. Since $\mathcal K^*(x, x')$ does not depend on $x$ or $x'$ it follows that $\chi(x, x')$ will take on a single value, $\chi_{c^*}$, whenever $x\neq x'$. If $\chi_{c^*} < 1$ then this $\mathcal{K^*}$ fixed point is stable, but if $\chi_{c^*} > 1$ then the fixed point is unstable and, as discussed above, the system will converge to a different fixed point. If $\chi_{c^*} = 1$ then the hyperparameters lie at a phase transition and convergence is non-exponential. As was shown in~\citet{poole2016exponential}, there is always a fixed-point at $c^* = 1$ whose stability is determined by $\chi_1$. This is the so-called ordered phase since any pair of inputs will converge to identical outputs. The line defined by $\chi_1=1$ defines the order-to-chaos transition separating the ordered phase from the ``chaotic'' phase (where $c^* > 1$). Note, that $\chi_{c^*}$ can be used to define a depth-scale, $\xi_{c^*} = -1 / \log(\chi_{c^*})$ that describes the number of layers over which $\Kl$ approaches $\mathcal K^*.$

This provides a precise characterization of the NNGP kernel at large depths. As discussed above, recent work~\citep{Jacot2018ntk, lee2019wide, chizat2019lazy} has connected the prior described by the NNGP with the result of gradient descent training using a quantity called the NTK. To construct the NTK, suppose we enumerate all the parameters in the fully-connected network described above by $\theta_\alpha$. The finite width NTK is defined by $\finntk(x, x') = J(x)J(x')^T$ where $J_{i\alpha}(x) = \partial_{\theta_\alpha}z^L_i(x)$ is the Jacobian evaluated at a point $x$. The main result in~\citet{Jacot2018ntk} was to show that in the infinite-width limit, the NTK converges to a deterministic kernel $\infntk$ and remains constant over the course of training. As such, at a time $t$ during gradient descent training with an MSE loss, the expected outputs of an infinitely wide network, $\mu_t(x) = \mathbb E[z^L_i(x)]$, evolve as
\begin{align}\label{eq:fc_ntk_recap_dynamics}
    \mu_t(X_{\text{train}}) &= (\Id - e^{-\eta\infntk_{\text{train, train}}t})Y_{\text{train}}
    \\
    \mu_t(X_{\text{test}}) &= \infntk_{\text{test, train}}\infntk_{\text{train, train}}^{-1}(\Id - e^{-\eta\infntk_{\text{train, train}}t})Y_{\text{train}}
    \label{eq:ntk-predictor} 
% \normalsize 
\end{align}
\normalsize
for train and test points respectively; see Section 2 in \citet{lee2019wide}. Here $\Theta_{\text{test, train}}$ denotes the NTK between the test inputs $X_{\text{test}}$ and training inputs $X_{\text{train}}$ and $\Theta_{\text{train, train}}$ is defined similarly. 
Since $\finntk$ converges to $\infntk$ as the network's width approaches infinity, the gradient flow dynamics of real network also converge to the dynamics described by \eqref{eq:fc_ntk_recap_dynamics} and \eqref{eq:ntk-predictor}
\citep{Jacot2018ntk, lee2019wide, chizat2019lazy, yang2019scaling, arora2019exact,huang2019dynamics}.  
As the training time, $t$, tends to infinity we note that these equations reduce to $\mu(X_{\text{train}}) = Y_{\text{train}}$ and $\mu(X_{\text{test}}) = \Theta_{\text{test, train}}\Theta_{\text{train, train}}^{-1} Y_{\text{train}}$. Consequently we call
\begin{align}\label{eq:linear-predictor} 
    P(\Theta) \equiv \Theta_{\text{test, train}}\Theta_{\text{train, train}}^{-1}
\end{align}
 the ``mean predictor''. We can also compute the mean predictor of the NNGP kernel, $P(\K)$, which analogously can be used to find the mean of the posterior after Bayesian inference. We will discuss the connection between the mean predictor and generalization in the next section.
 
 In addition to showing that the NTK describes networks during gradient descent, \citet{Jacot2018ntk} showed that the NTK could be computed in closed form in terms of $\mathcal T$, $\dot{\mathcal T}$, and the NNGP as,
\begin{equation}\label{eq: NTK-recursive}
 \scalebox{.9}{
$    \Thetall(x, x') = \Kll(x, x') + \sigma_w^2\dot{\T}(\Kl)(x, x')\Thetal(x, x')\,$.}
\end{equation}
where $\Thetal$ is the NTK for the pre-activations at layer-$l$. 
        \section{Metrics for Trainability and Generalization at Large Depth}
        We begin by discussing the interplay between the conditioning of $\Theta_{\text{train, train}}$ and the trainability of wide networks. We can write \eqref{eq:fc_ntk_recap_dynamics} in terms of the spectrum of $\Theta_{\text{train, train}}$. To do this we write the eigendecomposition of $\Theta_{\text{train, train}}$ as $\Theta_{\text{train, train}} = U^TDU$ with $D$ a diagonal matrix of eigenvalues and $U$ a unitary matrix. In this case \eqref{eq:fc_ntk_recap_dynamics} can be written as,
        \begin{equation}\label{eq:fc_ntk_dynamics_eigen}
        \tilde\mu_t(X_{\text{train}})_i = (\text{Id} - e^{-\eta \lambda_i t})\tilde Y_{\text{train},i}   
        \end{equation}
        where $\lambda_i$ are the eigenvalues of $\Theta_{\text{train, train}}$ and $\tilde\mu_t(X_{\text{train}}) = U\mu_t(X_{\text{train}})$, $\tilde Y_{\text{train}} = U Y_{\text{train}}$ are the mean prediction and the labels respectively written in the eigenbasis of $\Theta_{\text{train,train}}$. If we order the eigenvalues such that $\lambda_0 \geq \cdots \geq \lambda_m$ then it has been hypothesized\footnote{For finite width, the optimization problem is non-convex and there are not rigorous bounds on the maximum learning rate.} in e.g.~\citet{lee2019wide} that the maximum feasible learning rate scales as $\eta \sim 2 / \lambda_0$ as we verify empirically in section 4. Plugging this scaling for $\eta$ into \eqref{eq:fc_ntk_dynamics_eigen} we see that the smallest eigenvalue will converge exponentially at a rate given by $1/\kappa$, where $\kappa =  \lambda_0 / \lambda_m$ is the condition number.  It follows that if the condition number of the NTK associated with a neural network diverges then it will become untrainable and so we use $\kappa$ as a metric for trainability. 
        
        We will see that at large depths, the spectrum of $\Theta_{\text{train, train}}$ typically features a single large eigenvalue, $\lambda_{\text{max}}$, and then a gap that is large compared with the rest of the spectrum. We therefore will often refer to a typical eigenvalue in the bulk as $\lrest$ and approximate the condition number as $\kappa = \lambda_{\text{max}} / \lrest$.
        
        
        We now turn our attention to generalization. At large depths, we will see that $\Thetal_{\text{test, train}}$ and $\Thetal_{\text{train, train}}$ converge their fixed points independent of the data distribution. Consequently it is often the case that $P(\Theta^*)$ will be data-independent and the network will fail to generalize. In this case, by symmetry, it is necessarily true that $P(\Theta^*)$ will be a constant matrix. Contracting this matrix with a vector of labels $Y_{\text{train}}$ that have been standardized to have zero mean it will follow that $P(\Theta^*)Y_{\text{train}} = 0$ and the network will output zero in expectation on all test points. Clearly, in this setting the network will not be able to generalize. At large, but finite, depths the generalization performance of the network can be quantified by considering the rate at which $P(\Thetal)Y_{\text{train}}$ decays to zero. There are cases, however, where despite the data-independence of $\Theta^*$, $\lim_{l\to\infty} P(\Thetal)Y_{\text{train}}$ remains nonzero and the network can continue to generalize even in the asymptotic limit. In either case, we will show that precisely characterizing $P(\Thetal)Y_{\text{train}}$ allows us to understand exactly where networks can, and cannot, generalize.


        Our goal is therefore to characterize the evolution of the two metrics $\kappal$ and $\Deltal$ in $l$. We follow the methodology outlined in~\citet{schoenholz2016, xiao18a} to explore the spectrum of the NTK as a function of depth. We will use this to make precise predictions relating trainability and generalization to the hyperparameters $(\sigma_w, \sigma_b, l)$. Our main results are summarized in Table \ref{table evolution ntk} which describes the evolution of $\lmaxl$ (the largest eigenvalue of $\Thetal$), $\lrestl$ (the remaining eigenvalues), $\kappal$, and $\Deltal$ as a function of depth for three different network configurations (the ordered phase, the chaotic phase, and the phase transition). We study the dependence on: the size of the training set, $m$; the choices of architecture including fully-connected networks (FCN), convolutional networks with flattening (CNN-F), and convolutions with pooling (CNN-P); and the size, $d$, of the window in the pooling layer (which we always take to be the penultimate layer).
        
        Before discussing the methodology it is useful to first give a qualitative overview of the phenomenology. We find identical phenomenology between FCNs and CNN-F architectures. In the ordered phase, $\Thetal\to \pstar \bm1 \bm1^T$, $\lmaxl\to mp^*$ and $\lrestl=\bigo (l\chi_1^l)$. At large depths since $\chi_1 < 1$ it follows that $\kappal\gtrsim mp^* / (l\chi_1^l)$ and so the condition number diverges exponentially quickly. Thus, in the ordered phase we expect networks not to be trainable (or, specifically, the time they take to learn will grow exponentially in their depth). Here $\Deltal$ converges to a data dependent constant independent of depth; thus, in the ordered phase networks fail to train but can generalize indefinitely. 
        
        By contrast, in the chaotic phase we see that there is no gap between $\lmaxl$ and $\lrestl$ and networks become perfectly conditioned and are trainable everywhere.  However, in this regime we see that the mean predictor scales as $l (\chi_{c^*} / \chi_1)^l$. Since in the chaotic phase $\chi_{c^*} < 1$ and $\chi_1 > 1$ it follows that $\Deltal\to 0$ over a depth $\xi_{*} = -1/\log(\chi_{c^*} / \chi_1)$. Thus, in the chaotic phase, networks fail to generalize at a finite depth but remain trainable indefinitely. Finally, introducing pooling modestly augments the depth over which networks can generalize in the chaotic phase but reduces the depth in the ordered phase. We will explore all of these predictions in detail in section~\ref{sec:experiments}.
        

==> Trainability-Generalization-ICML2020 (2)/tex_zoo/intro.tex <==

\section{Introduction}

Machine learning models based on deep neural networks have attained state-of-the-art performance across a dizzying array of tasks including vision~\citep{cubuk2019}, speech recognition~\citep{park2019}, machine translation~\citep{bahdanau2014}, chemical property prediction~\citep{gilmer2017}, diagnosing medical conditions~\citep{raghu2019}, and playing games~\citep{silver1140}. Historically, the rampant success of deep learning models has lacked a sturdy theoretical foundation: architectures, hyperparameters, and learning algorithms are often selected by brute force search~\citep{bergstra2012} and heuristics~\citep{glorot2010understanding}. Recently, significant theoretical progress has been made on several fronts that have shown promise in making neural network design more systematic. In particular, in the infinite width (or channel) limit, the distribution of functions induced by neural networks with random weights and biases has been precisely characterized before, during, and after training.

The study of infinite networks dates back to seminal work by~\citet{neal} who showed that the distribution of functions given by single hidden-layer networks with random weights and biases in the infinite-width limit are Gaussian Processes (GPs). Recently, there has been renewed interest in studying random, infinite, networks starting with concurrent work on ``conjugate kernels''~\citep{daniely2016, daniely2017sgd} and ``mean-field theory''~\citep{poole2016exponential,schoenholz2016}. Among numerous contributions, the pair of papers by Daniely \textit{et al.} argued that the empirical covariance matrix of pre-activations becomes deterministic in the infinite-width limit and called this the conjugate kernel of the network. Meanwhile, from a mean-field perspective, the latter two papers studied the properties of these limiting kernels. In particular, the spectrum of the conjugate kernel of wide, fully-connected, networks approaches a well-defined and data-independent limit when the depth exceeds a certain scale, $\xi$. Networks with $\tanh$-nonlinearities (among other bounded activations) exhibit a phase transition between two limiting spectral distributions of the conjugate kernel as a function of their hyperparameters with $\xi$ diverging at the transition. It was additionally hypothesized that networks were un-trainable when the conjugate kernel was sufficiently close to its limit. 

Since then this analysis has been extended to include a wide range for architectures such as convolutions~\citep{xiao18a}, recurrent networks~\citep{chen2018rnn, gilboa2019}, networks with residual connections~\citep{yang2017}, networks with quantized activations~\citep{blumenfeld2019}, the spectrum of the fisher~\citep{karakida2018universal}, a range of activation functions~\citep{hayou2018selection}, and batch normalization~\citep{yang2019mean}. In each case, it was observed that the spectra of the kernels correlated strongly with whether or not the architectures were trainable. While these papers studied the properties of the conjugate kernels, especially the spectrum in the large-depth limit, a branch of concurrent work took a Bayesian perspective: that many networks converge to Gaussian Processes as their width becomes large~\citep{lee2018deep, matthews2018, novak2018bayesian, garrigaalonso2018deep, yang2019scaling}. In this case, the Conjugate Kernel was referred to as the Neural Network Gaussian Process (NNGP) kernel, which is used to train neural networks in a fully Bayesian fashion. As such, the NNGP kernel characterizes performance of the corresponding NNGP.    

Together this work offered a significant advance to our understanding of wide neural networks; however, this theoretical progress was limited to networks at initialization or after Bayesian posterior estimation and provided no link to gradient descent. Moreover, there was some preliminary evidence that suggested the situation might be more nuanced than the qualitative link between the NNGP spectrum and trainability might suggest. For example,~\citet{philipp2017exploding} showed that deep $\tanh$ FCNs could be trained after the kernel reached its large-depth, data-independent, limit but that these networks did not generalize to unseen data. 

Recently, significant theoretical clarity has been reached regarding the relationship between the GP prior and the distribution following gradient descent. In particular,~\citet{Jacot2018ntk} along with followup work~\citep{lee2019wide, chizat2019lazy} showed that the distribution of functions induced by gradient descent for infinite-width networks is a Gaussian Process with a particular compositional kernel known as the Neural Tangent Kernel (NTK). In addition to characterizing the distribution over functions following gradient descent in the wide network limit, the learning dynamics can be solved analytically throughout optimization.


In this paper, we leverage these developments and revisit the relationship between architecture, hyperparameters, trainability, and generalization in the large-depth limit for a variety of neural networks. In particular, we make the following contributions:
\begin{itemize}
    \item {\bf Trainability.} We compute the large-depth asymptotics of several quantities related to trainability, including the largest/smallest eigenvalue of the NTK, $\lambda_{\text{max}/\text{min}}$, and the condition number $\kappa = \lambda_{\text{max}}/\lambda_{\text{min}}$; see Table~\ref{table evolution ntk}. 

    \item {\bf Generalization.} We characterize the {\it mean predictor} $P(\Theta)$, which is intimately related to the prediction of wide neural networks on the test set following gradient descent training. As such, the mean predictor is intimately related to the model's ability to generalize. In particular, we argue that networks fail to generalize if the mean predictor becomes data-independent.
    % We will quantify this breakdown by contracting the mean predictor with mean centered labels $P(\Theta)Y_{\text{train}}$.

    \item We show that the \emph{ordered} and \emph{chaotic} phases identified in~\citet{poole2016exponential} lead to markedly different limiting spectra of the NTK. In the ordered phase the trainability of neural networks degrades at large depths, but their ability to generalize persists. By contrast, in the chaotic phase we show that trainability improves with depth, but generalization degrades and neural networks behave like hash functions.
    
    A corollary of these differences in the spectra is that, as a function of depth, the optimal learning rates ought to decay exponentially in the chaotic phase, linearly on the order-to-chase trainsition line, and remain roughly a constant in the ordered phase.
    \item We examine the differences in the above quantities for fully-connected networks (FCNs) and convolutional networks (CNNs) with and without pooling and precisely characterize the effect of pooling on the interplay between trainability, generalization, and depth.
\end{itemize}


In each case, we provide empirical evidence to support our theoretical conclusions. Together these results provide a complete, analytically tractable, and dataset-independent theory for learning in very deep and wide networks. Philosophically, we find that trainability and generalization are distinct notions that are, at least in this case, at odds with one another. Indeed, good conditioning of the NTK (which is a necessary condition for training) seems necessarily to lead to poor generalization performance. It will be interesting to see whether these results carry over in shallower and narrower networks. The tractable nature of the wide and deep regime leads us to conclude that these models will be an interesting testbed to investigate various theories of generalization in deep learning. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llll}
        \toprule
                  & \multicolumn{3}{c}{{\color[HTML]{000000} NTK $\Thetal$ of  FC/CNN-F, \quad  \color{blue}{CNN-P}}}\\[0.1cm]  
        \midrule
\multirow{-2}{*}{}  & Ordered     $\chi_1 <1$       & Critical $\chi_1=1$            & Chaotic $\chi_1 > 1$            \\ [0.4cm]
                 $ \lmaxl$                 &   $m\pstar +m \bigo (l\chi_1^l)$        &       $\frac {m{\colord} +2} {3\colord} l\qstar   + m \bigo(1)$         &      $\Theta(\chi_1^l)\color{blue}{/}\colord$  \\ [0.4cm]
                  $\lrestl$                 &  $ \bigo(l\chi_1^l)\color{blue}{/}\colord$          &     $\frac 2 {3 \colord } l\qstar  + \frac{1}{\colord}\bigo(1)$          &            $\Theta(\chi_1^l)\color{blue}{/}\colord$                  \\ [0.4cm]
                  $\kappal$                 &   $\colord m\pstar \Omega(\chi_1^{-l} / l)$         
                  &    $\frac {m{\colord} +2} 2 + \colord  m\bigo(l^{-1})$            & $1 + \bigo({\colord}\chi_1^{-l})$                
                  \\ [0.4cm]
                  $P(\Thetal)Y_{\text{train}}$                 &   $ \bigo(1)$         
                  &    $\colord  \bigo(l^{-1})$            
                  & $\colord \bigo(l (\chi_{c^*}/\chi_1)^l  )$            
                  \\
        \bottomrule
\end{tabular}% 
} 
\end{center}
\captionsetup{singlelinecheck=off}
    \caption{\textbf{Evolution of the NTK spectra and $\Deltal$ as a function of depth $l$.} The NTKs of FCN and CNN without pooling (CNN-F) are essentially the same and the scaling of $\lmaxl$, $\lrestl$, $\kappal$, and $\Delta^{(l)}$ for these networks is written in black. Corrections to these quantities due to the addition of an average pooling layer ({\color{blue} CNN-P}) with window size $\colord$ is written in blue.}
    \label{table evolution ntk}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Trainability-Generalization-ICML2020 (2)/tex_zoo/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% \newcommand{\Id}{{\text{Id}}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}
\newcommand{\colord}{{\color{blue}{d}}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
\def\eqref#1{\Eqref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\DKL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\usepackage{subcaption}
\usepackage{bbm}
\usepackage{bm}
\usepackage{mathtools}
\usepackage{amsthm, amssymb}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{claim}{Claim}[theorem]
\newtheorem{corollary}{Corollary}%[section]
\newtheorem{remark}{Remark}%[section]



\def\1{\bm{1}}
\newcommand{\D}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\flin}{f^{\textrm{lin}}}
\newcommand{\glin}{g^{\textrm{lin}}}
\newcommand{\dflin}{{{\dot f}_t^{\textrm {lin}}}}
\newcommand{\dglin}{{{\dot g}_t^{\textrm {lin}}}}
\newcommand{\Llin}{L^{\textrm{lin}}}
\newcommand{\ly}{{\ell_{\hat y}}} 
\newcommand{\chic}{\chi_{c^*}}

\newcommand{\N}{\mathcal N}
\newcommand{\bparam}{\mu}
\newcommand{\flatten}{\mathcal F}
\newcommand{\pool}{\mathcal P}
\newcommand{\h}{y}
\newcommand{\hatthetal}{{\hat \Theta}^{(l)}}
\newcommand{\A}{\mathcal A}
\newcommand{\nin}{n_{in}}
\newcommand{\nout}{n_{out}}
\newcommand{\dotphi}{\dot\phi}
\newcommand{\Id}{\textbf{Id}} 
\newcommand{\sw}{\sigma_\omega}
\newcommand{\sws}{\sigma_\omega^2}
\newcommand{\sbb}{\sigma_b}
\newcommand{\sbs}{\sigma_b^2}
\newcommand{\ql}{q^{(l)}}
\newcommand{\pl}{p^{(l)}}
\newcommand{\pll}{p^{(l+1)}}
\newcommand{\qll}{q^{(l+1)}}
\newcommand{\elab}{\epsilon_{ab}^{(l)}}
\newcommand{\dlab}{\delta_{ab}^{(l)}}
\newcommand{\ellab}{\epsilon_{ab}^{(l+1)}}
\newcommand{\dllab}{\delta_{ab}^{(l+1)}}
\newcommand{\elaba}{\epsilon_{ab,\alpha}^{(l)}}
\newcommand{\dlaba}{\delta_{ab, \alpha}^{(l)}}
\newcommand{\ellaba}{\epsilon_{ab, \alpha}^{(l+1)}}
\newcommand{\dllaba}{\delta_{ab, \alpha}^{(l+1)}}
\newcommand{\cstar}{c^{*}}

\newcommand{\pstar}{p^{*}}
\newcommand{\pabstar}{p_{ab}^{*}} 
\newcommand{\pabl}{p^{(l)}_{ab}}
\newcommand{\qabl}{q^{(l)}_{ab}}
\newcommand{\qabstar}{q^{*}_{ab}}
\newcommand{\pabll}{p^{(l+1)}_{ab}}
\newcommand{\qabll}{q^{(l+1)}_{ab}}
\newcommand{\bigo}{\mathcal {O}}
\newcommand{\lmax}{\lambda_{\rm max}}
\newcommand{\lmaxl}{\lambda_{\rm max}^{(l)}}
\newcommand{\lmin}{\lambda_{\rm min}}
\newcommand{\lrest}{\lambda_{\rm bulk}}
\newcommand{\lrestl}{\lambda_{\rm bulk}^{(l)}}
\newcommand{\kappal}{\kappa^{(l)}}
\newcommand{\Thetalft}{\Thetal_{\rm flatten}}
\newcommand{\Thetalpool}{\Thetal_{\rm pool}}

\newcommand{\norm}[1]{\lVert #1 \rVert}
% \newcommand{\norm}[1]{\left|\left| #1 \right|\right|}
\newcommand{\dd}{{\mathrm{d}}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdn}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}
\newcommand{\od}[2]{\frac{\dd #1}{\dd #2}}
\newcommand{\odn}[3]{\frac{\dd^#1 #2}{\dd #3^#1}}
\newcommand{\avg}[1]{\left< #1 \right>}
\newcommand{\pp}[1]{\left( #1 \right)}
\newcommand{\mb}{\mathbf}
\newcommand{\mx}{\mathbf x}
\newcommand{\mc}{\mathcal}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\median}{\operatornamewithlimits{median}}
\newcommand{\expect}[2]{\mathbbm{E}_{#1}\left[ #2 \right]}
\newcommand{\finntk}{\hat\Theta}
\newcommand{\infntk}{\Theta}
\newcommand{\infnngp}{\mathcal K}
\newcommand{\finnngp}{\hat {\mathcal K}}
\newcommand{\tpoint}{x}
\newcommand{\Kl}{\mathcal K^{(l)}}
\newcommand{\Klft}{\mathcal K^{(l)}_{\rm flatten}}
\newcommand{\Klpool}{\mathcal K^{(l)}_{\rm pool}}
% \newcommand{\Thetalfc}{\mathcal T^{(l)}_{\rm fc}}
\newcommand{\Thetalfc}{\Thetal_{\rm fc}}

% \newcommand{\Deltal}{\Delta^{(l)}}
\newcommand{\Deltal}{P(\Thetal)}
\newcommand{\Kll}{\mathcal K^{(l+1)}}
\newcommand{\Thetal}{ \Theta^{(l)}}
\newcommand{\Thetall}{\Theta^{(l+1)}} 
\newcommand{\el}{\epsilon^{(l)}} 
\newcommand{\elll}{\epsilon^{(l+1)}} 
\newcommand{\dll}{\delta^{(l+1)}} 
\newcommand{\dl}{\delta^{(l)}} 
\newcommand{\pab}{p^*_{ab}}
\newcommand{\qab}{q^*_{ab}}
\newcommand{\op}{\rm{op}}
\newcommand{\mins}{\lambda_{\rm{min}}}
\newcommand{\maxs}{\lambda_{\rm{max}}}
\newcommand{\q}{\quad}
\newcommand{\lss}{R_0}
\newcommand{\GP}{\mc {GP}}
\newcommand{\relu}{{$\operatorname{ReLU}$}}
\newcommand{\erf}{$\operatorname{erf}$ }
\newcommand{\critical}{\eta_{{\rm critical}} }
\newcommand{\Aop}{ {\mathcal A} \ast}
\newcommand{\dT}{\dot \T}
\newcommand{\qstar}{q^{*}} 
\newcommand{\Ytest}{Y_{\text{test}}} 
\newcommand{\Ytrain}{Y_{\text{train}}} 
\newcommand{\gammal}{\gamma^{(L)}}
\newcommand{\NL}{N^{(L)}}
\newcommand{\WL}{W^{(L+1)}}
\newcommand{\KL}{\K^{(L)}}
\newcommand{\KLL}{\K^{(L+1)}}

% \newcommand{\norm}[1]{\lVert #1 \rVert}
% % \newcommand{\norm}[1]{\left|\left| #1 \right|\right|}
% \newcommand{\dd}{{\mathrm{d}}}
% \newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
% \newcommand{\pdn}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}
% \newcommand{\od}[2]{\frac{\dd #1}{\dd #2}}
% \newcommand{\odn}[3]{\frac{\dd^#1 #2}{\dd #3^#1}}
% \newcommand{\avg}[1]{\left< #1 \right>}
% \newcommand{\pp}[1]{\left( #1 \right)}
% \newcommand{\mb}{\mathbf}
% \newcommand{\mx}{\mathbf x}
% \newcommand{\mc}{\mathcal}


==> Trainability-Generalization-ICML2020 (2)/tex_zoo/theory_experiments.tex <==

       
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% condition number plots 

\begin{figure*}[t] 
\begin{center}
         \begin{subfigure}[b]{.33\textwidth}
                \centering
\includegraphics[width=1.\textwidth]{new_graphs/graphs-test/Condition-number-ALL-Chaotic-NTK.pdf}
                \caption{Chaotic}
                \label{fig:kappa-chaotic}
        \end{subfigure}
        \begin{subfigure}[b]{0.33\textwidth}
                \centering
               \includegraphics[width=1\textwidth]{new_graphs/graphs-test/Condition-number-ALL-Ordered-NTK.pdf}
                \caption{Ordered}
                \label{fig:kappa-order}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\textwidth}
                \centering
\includegraphics[width=1.\textwidth]{new_graphs/graphs-test/Condition-number-FC-CNN-F-Critical-NTK-with-dashed.pdf}
                \caption{Critical: FCN and CNN-F}
                \label{fig:kappa-critical}
        \end{subfigure}%
        \\ 
 \begin{subfigure}[b]{0.33\textwidth}
                \centering
     \includegraphics[width=1.\textwidth]{new_graphs/graphs-test/condition-number-critical-p-0.pdf}
                \caption{Critical: CNN-P}
                \label{fig:kappa-cnn-p}
        \end{subfigure}%
        \begin{subfigure}[b]{0.33\textwidth}
                \centering
              \includegraphics[width=1.\textwidth]{new_graphs/generalization_plots/generalization-chaotic-lw.pdf}
                \caption{Chaotic: $P(\Thetal)Y_{\text{train}}$}
                \label{fig:mean-pred-chaotic}
        \end{subfigure}%
 \begin{subfigure}[b]{0.33\textwidth}
                \centering
          \includegraphics[width=1.\textwidth]{new_graphs/generalization_plots/generalization-ordered-logx-lw.pdf}
                \caption{Ordered: $P(\Thetal)Y_{\text{train}}$}
                \label{fig:mean-pred-ordered}
        \end{subfigure}%
\end{center}
\caption{{\bf Condition number and mean predictor of NTKs and their rate of convergence for FCN, CNN-F and CNN-P.}
(a) In the chaotic phase, $\kappal$ converges to 1 for all architectures. 
(b) We plot $\chi_1^l\kappal$, confirming that
 $\kappa$ explodes with rate $1/l\chi_1^l$ in the ordered phase. 
In (c) and (d), the solid lines are $\kappal$ and dashed lines are the ratio between first and second eigenvalues. We see that, on the order-to-chaos transition,  these two numbers converge to $\frac {m+2}{2}$ and $\frac{dm+2}{2}$ (horizontal lines) for FC/CNN-F and CNN-P respectively, where $m=12$ or $20$ is the batch size and $d=36$ is the spatial dimension. 
(e) In the chaotic phase, the mean predictor decays to zero exponentially fast. (f) In the ordered phase the mean predictor converges to a data dependent value. 
}
\label{fig: conditioning-complete}
\end{figure*}
\section{A Toy Example: RBF Kernel}
To provide more intuition about our analysis, we present a toy example using RBF kernels which already shares some core observations for deep neural networks. Consider a Gaussian process along with the RBF kernel given by,
\begin{align}
    K_h(x, x') = \exp\left(-\frac{\|x - x'\|^2_2}{h}\right) 
\end{align}
where $x, x' \in X_{\text{train}}$ along with a bandwidth $h>0$. Note that $K_h(x, x)=1$ for all $h$ and $x$. Considering the following two cases.

If the bandwidth is given by $h=2^l$ and $l\to\infty$, then $K_h(x, x') \approx 1 - 2^{-l}\|x - x'\|^2_2$ which converges to $1$ exponentially fast. Thus, the largest eigenvalue of $K_h$ is $\lambda_{\text{max}}\approx|X_{\text{train}}|$ and the bulk is of order $\lambda_{\text{bulk}}\approx 2^{-l}$. Thus the condition number $\kappa \gtrsim 2^l$ which diverges with $l$. We will see in the \textbf{Ordered Phase} $\Thetal$ behaves qualitatively similar to this setting. 
    
On the other hand, if the bandwidth is given by $h=1/l$ and $l\to \infty$ then the off-diagonals $K_h(x, x') = \exp(-l \|x-x'\|_2^2)\to 0 $. For large $l$, $K_h$ is very close to the identity matrix and the condition number of it is almost 1. In the \textbf{Chaotic Phase}, $\Thetal$ is qualitatively similar to $K_h$.     
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \section{Large-Depth Asymptotics of the NNGP and NTK}
        \label{sec:theory} 
        We now give a brief derivation of the results in Table~\ref{table evolution ntk}. Details can be found in Sec.\ref{sec:signal-propagation}, \ref{sec:deltal} in the appendix. To simplify notation we will discuss fully-connected networks and then extend the results to CNNs with pooling (CNN-P) and without pooling (CNN-F). 
        
        As in Sec.~\ref{sec:background}, we will be concerned with the fixed points of $\Theta$ as well as the linearization of ~\eqref{eq: NTK-recursive} about its fixed point.
        Recall that the fixed point structure is invariant within a phase so it suffices to consider the ordered phase, the chaotic phase, and the critical line separately. In cases where a stable fixed point exists, we will describe how $\Theta$ converges to the fixed point. We will see that in the chaotic phase and on the critical line, $\Theta$ has no stable fixed point and in that case we will describe its divergence. As above, in each case the fixed points of $\Theta$ have a simple structure with $\Theta^* = p^* ((1- \hat c^{*}) \Id  + \hat c^{*}\1 \1^T)$.  
        
        To simplify the forthcoming analysis, without a loss of generality, we assume the inputs are normalized to have variance $q^*$ \footnote{It has been observed in previous works \citep{poole2016exponential, schoenholz2016} that the diagonals converge much faster than the off-diagonals for $\tanh$- or erf- networks.}. As such, we can treat $\T$ and $\dT$, restricted on $\{\Kl\}_{l}$, as a point-wise functions. To see this note that with this normalization $\K^{(l)}(x, x)=q^*$ for all $l$ and $x$. It follows that both $\T(\Kll)(x, x')$ and $\dT(\Kll)(x,x')$ depend only on $\Kl(x,x')$.  
        
        Since all of the off-diagonal elements approach the same fixed point at the same rate, we use $\qabl \equiv\Kl(x, x')$ and $\pabl\equiv\Thetal(x,x')$ to denote any off diagonal entry of $\Kl$ and $\Thetal$ respectively. We will similarly use $\qabstar$ and $\pabstar$ to denote the limits, $\lim_{l\to\infty}\qabl = \qabstar =c^*\qstar$ and $\lim_{l\to\infty}\pabl = \pabstar = \hat c^* \pstar$. Finally, although the diagonal entries of $\Kl$ are all $q^*$, the diagonal entries of $\Thetal$ can vary and we denote them $\pl$.
        
        In what follows, we split the discussion into three sections according to the values of $\chi_1 \equiv \sws\dot\T(q^*) $ recalling that in \citet{poole2016exponential, schoenholz2016} it was shown that $\chi_1$ controls the fixed point structure. In each section, we analyze the evolution of (1) the entries of $\Thetal$, i.e., $\pl$, $\pabl$, (2) the spectrum $\lmaxl$ and $\lrestl$, (3) the trainability and generalization metrics $\kappal$ and $\Deltal$, and finally (4) discuss the impact on finite width networks. 
        %The deviation for all the results are be found in Sec.~\ref{sec:signal-propagation} and ~\ref{sec:deltal}. 
        
\subsection{The Chaotic Phase $\chi_1 > 1$:}
The chaotic phase is so-named because it has a stable fixed-point $c^* < 1$; as such similar inputs become increasingly uncorrelated as they pass through the network. Our first result is to show that (see Sec.~\ref{sec:signal-prog-chaotic}), 
\small 
\begin{align}
    \begin{cases}
    \qabl = \qabstar + \bigo(\chic^l)
    \\
    \ql = \qstar
    \end{cases}
    \begin{cases}
        \pabl = \pabstar + \bigo(l\chic^l)
        \\
        \pl =  q^* \frac {\chi_1^{l} - 1} {\chi_1 - 1 }
    \end{cases}
\end{align}
\normalsize 
where 
\begin{align}
    \pabstar = \qabstar /(1 -\chic) \,\,\,{\rm and}\,\,\, \chic = \sws \dot \T(\qabstar)
\end{align}
Note that $\chic$ controls the convergence of the $\qabl$ and is always less than 1 in the chaotic phase ~\citep{poole2016exponential, schoenholz2016, xiao18a}. Since $\chi_1 > 1$, $\pl$ diverges with rate $\chi_1^l$ while $\pabl$ remains finite. It follows that $(\pl)^{-1}\Thetal \to \Id$ as $l\to\infty$. Thus, in the chaotic phase, the spectrum of the NTK for very deep networks approaches the diverging constant multiplying the identity. This implies 
\begin{align*}
\lmaxl, \, \lrestl = \pl + O(1) \,\,  {\rm and} \,\, \kappal = 1 + \bigo\left(\frac1 {\pl}\right)
\end{align*}
Figure~\ref{fig:kappa-chaotic} plots the evolution of $\kappal$ in this phase, confirming $\kappal \to 1$ for all three different architectures (FCN, CNN-F and CNN-P).

We now describe the asymptotic behavior of the mean predictor. Since $\Theta_{\text{test, train}}^l$ has no diagonal elements, it follows that it remains finite at large depths and so $P(\Theta^*) \Ytrain = 0$. It follows that in the chaotic phase, the predictions of asymptotically deep neural networks on unseen test points will converge to zero exponentially quickly (see Sec.~\ref{sec:deltal-chaotic}),
\begin{align}\label{eq:chaotic-solution}
\Deltal Y_{\text{train}} \approx
\bigo(l(\chic/\chi_1)^l)\to \bf 0.  
\end{align}
Neglecting the relatively slowly varying polynomial term, this implies that we expect chaotic networks to fail to generalize when their depth is much larger than a scale set by $\xi_* = -1 / \log(\chic/\chi_1)$. We confirm this scaling in Fig~\ref{fig:mean-pred-chaotic}.

We confirm these predictions for finite-width neural network training using SGD as well as gradient-flow on infinite networks in the experimental results; see Fig~\ref{fig:pool vs flatten}.


\subsection{The Ordered Phase $\chi_1 = \sws  \dot \T (q^*)  < 1$:}
The ordered phase is defined by the stability of the $c^* = 1$ fixed point. Here disparate inputs will end up converging to the same output at the end of the network. We show in Sec.~\ref{sec:signal-prog-ordered} that elements of the NNGP kernel and NTK have asymptotic dynamics given by, 
\begin{align}\label{eqn:signal-prop-ordered-main}
    \begin{cases}
    \qabl = \qstar  + \bigo(\chi_1^l)
    \\ 
    \ql = \qstar 
    \end{cases}
    \begin{cases}
    \pabl = \pstar + \bigo(l\chi_1^l) 
    \\
    \pl = \pstar + \bigo(\chi_1^l) 
    \end{cases}
\end{align}
where $\pstar = \qstar / (1 - \chi_1)$. Here all of the entries of $\Thetal$ converge to the same value, $\pstar$, and the limiting kernel has the form  
    $\Theta^* = p^*  \bf{1}_n\bf{1}_m^T$ where $\bf{1_m}$ is the all-ones vector of dimension $m$ (typically $m$ will correspond to the number of datapoints in the training set). The NNGP kernel has the same structure with $p^*\leftrightarrow q^*$.
    Consequently both the NNGP kernel and the NTK are highly singular and feature a single non-zero eigenvalue, $\lambda_{\text{max}} = mp^*$, with eigenvector $\bf{1_m}$.

For large-but-finite depths, $\Thetal$ has (approximately) two eigenspaces: the first eigenspace corresponds to finite-depth corrections to $\lambda_{\text{max}}$, 
\begin{align}
\lmaxl \approx (m-1) \pabl + \pl =  m\pstar + \bigo(l\chi_1^l).
\end{align} 
The second eigenspace comes from lifting the degenerate zero-modes has dimension $(m-1)$ with eigenvalues that scale like 
$
\lrestl = \bigo(\pl -\pabl) = \bigo(l\chi_1^{l}). 
$
It follows that $\kappal \gtrsim (l\chi_1^l)^{-1}$ and so the conditioning number explodes exponentially quickly. We confirm the presence of the $1/l$ correction term in $\kappal$ by plotting $\chi_1^l\kappal$ against $l$ in Figure~\ref{fig:kappa-order}. Neglecting this correction, we expect networks in the ordered phase to become untrainable when their depth exceeds a scale given by $\xi_1 = -1 / \log\chi_1$.

We now turn our discussion to the mean predictor. \eqref{eqn:signal-prop-ordered-main} shows that we can write the finite-depth corrections to the NTK as $\Thetal = p^* {\bf 1 1}^T + \bm{A}^{(l)} l\chi_1^l$. Here ${\bm A}^{(l)}$ is the data-dependent piece that lifts the zero eigenvalues. In the appendix, $\bm {A}^{(l)}$ converges to $\bm A$ as $l\to\infty$; see Lemma \ref{lemma:ordered}. 
In Sec.~\ref{sec:ordered-phase-mean-predictor} we show that despite the singular nature of $\Theta^*$, the mean has a well-defined limit as,
% could be approximately written as 
\begin{equation}
    \lim_{l\to\infty}P(\Thetal)Y_{\text{train}} = (\bm{A}_{\text{test, train}}\bm{A}_{\text{train, train}}^{-1} +\hat {\bm A})Y_{\text{train}},
\end{equation}
where $\hat {\bm A}$ is some correction term. Thus, the mean predictor remains well-behaved and data dependent even in the infinite-depth limit.
% We demonstrate the asymptotic data dependence of $\Deltal$ in Figure~\ref{fig:kappa-order}. 
Thus, we suspect that networks in the ordered phase should be able to generalize whenever they can be trained.  We confirm the asymptotic data-dependence of the mean predictor in Fig~\ref{fig:mean-pred-ordered}.


\subsection{The Critical Line $\chi_1 = \sws  \dot \T (q^*)  = 1$}
On the critical line the $c^* = 1$ fixed point is marginally stable and dynamics become powerlaw. Here, both the diagonal and the off-diagonal elements of $\Thetal$ diverge linearly in the depth with $\frac 1 l\Thetal\to \frac {\qstar} 3 (\bm 1\bm 1^T + 2 \Id)$. The condition number $\kappal$ converges to a finite value and the network is always trainable. However, the mean predictor decreases linearly with depth. In particular we show in Sec.~\ref{sec:signal-prog-critical}, 
\begin{align}
    \begin{cases}
    \qabl = \qstar  + \bigo(\frac 1 l)
    \\ 
    \ql = \qstar 
    \end{cases}
    \begin{cases}
    \pabl = \frac 1 3l \pstar + \bigo(1) 
    \\
    \pl = l \pstar 
    \end{cases}
\end{align}
For large $l$ it follows that $\Thetal$ essentially has two eigenspaces: one has dimension one and the other has dimension $(m-1)$ with 
\small 
\begin{align}
    \lmaxl = \frac {(m+2)q^*l} 3 + \bigo(1),  \,\,
  \lrestl = \frac {2q^* l} 3  +  \bigo(1).
\end{align}
\normalsize
It follows that the condition number $\kappal = \frac {m+2} 2 + m\bigo(l^{-1}) \to \frac {m+2} 2$ as $l\to\infty$. Unlike in the chaotic and ordered phases, here $\kappal$ converges with rate $\bigo(l^{-1})$. Figure~\ref{fig:kappa-critical} confirms the $\kappal\to  \frac {m+2} 2$ for both FCN and CNN-F (the global average pooling in CNN introduces a correction term that we will discuss below). A similar calculation gives $\Deltal = \bigo(l^{-1})$ on the critical line.

In summary, $\kappal$ converges to a finite number and the network ought to be trainable for arbitrary depth but the mean predictor $\Deltal$ decays as a powerlaw. Decay as $l^{-1}$ is much slower than exponential and is slow on the scale of neural networks. This explains why critically initialized networks with thousands of layers could still generalize~\citep{xiao18a}. 

\subsection{The Effect of Convolutions}
The above theory can be extended to CNNs. We will provide an informal description here, with details in Sec.~\ref{sec:conv-ntk}. For an input-images of size $(m, k, k, 3)$ the NTK and NNGP kernels will have shape $(m, k, k, m, k, k)$ and will contain information about the covariance between each pair of pixels in each image. For convenience we will let $d = k^2$. In the large depth setting deviations of both kernels from their fixed point decomposes via Fourier transform in the spatial dimensions as,
%the NTK of CNNs without pooling is essentially the same as the NTK of FCNs.
%Indeed, naively 
\begin{align}
    \delta \Thetal_{\rm CNN} \approx \sum_{q} \rho_q^l \delta \Thetal(q)
\end{align}
where $q$ denotes the Fourier mode with $q = 0$ being the zero-frequency (uniform) mode and $\rho_q$ are eigenvalues of certain convolution operator. Here $\delta\Thetal(q)$ are deviations from the fixed-point for the $q$\textsuperscript{th} mode with $\delta\Thetal(q)\propto \delta\Thetal_{\text{FCN}}$ the fully-connected deviation described above. We show that $\rho_{q=0} = 1$ and $|\rho_{q\neq 0}|<1$ which implies that asymptotically the nonuniform modes become subleading as  $\rho_{q}^l\to 0$. Thus, at large depths different pixels evolve identically as FCNs.

In Sec.~\ref{sec:cnn-pooling} we discuss the differences that arise when one combines a CNN with a flattening layer compared with an average pooling layer at the readout. In the case of flattening, the pixel-pixel correlations are discarded and $\Thetal_{\rm CNN-F} \approx \Thetal_{\rm FCN}$. The plots in the first row of Figure~\ref{fig: conditioning-complete} confirm that the $\kappal$ of $\Thetal_{\rm CNN-F}$ and of $\Thetal_{\rm FCN}$ evolve almost identically in all phases.  Note that this clarifies an empirical observation in \citet{xiao18a} (Figure 3 of \citet{xiao18a}) that test performance of critically initialized CNNs degrades towards that of FCNs as depth increases. This is because (i) in the large width limit, the prediction of neural networks is characterized by the NTK and (ii)
the NTKs of the two models are almost identical for large depth. However, when CNNs are combined with global average pooling a correction to the spectrum of the NTK (NNGP) emerges oweing to pixel-pixel correlations; this alters the dynamics of $\kappal$ and $\Deltal$. In particular, we find that global average pooling increases $\kappal$ by a factor of $d$ in the ordered phase and on the critical line; see Table~\ref{table evolution ntk} for the exact correction as well as Figures~\ref{fig:kappa-cnn-p} for experimental evidence of this correction.   

\subsection{Dropout, Relu and Skip-connection} 
% copy version; add pooling experiments. 
% move to section 6. 

Adding a dropout to the penultimate layer has a similar effect to adding a diagonal regularization term to the NTK, which significantly improves the conditioning of the NTK in the ordered phase. In particular, adding a single dropout layer can cause $\kappal$ to converge to a finite $\kappa^*$ rather than diverges exponentially; see Figure~\ref{fig:kappa-dropout} and Sec.~\ref{sec:dropout}.  
 
For critically initialized Relu networks (aka, He's initialization \cite{HeZR015}), the entries of the NTK also diverges linearly and $\kappal\to \frac{m+3}{3}$ and $\Deltal=\bigo(1/l)$; see Table~\ref{table evolution NTK-NNGP} and Figure~\ref{fig: conditioning-complete-NNGP}. In addition, adding skip-connections makes all entries of the NTK to diverge exponentially, resulting exploding of gradients. However, we find that skip connections do not alter the dynamics of $\kappal$. Finally, layer normalization could help address the issue of exploding of gradients; see Sec. \ref{sec:RElu-networks}.  


\section{Experiments}\label{sec:experiments}

{\bf Evolution of $\kappal$ (Figure~\ref{fig: conditioning-complete}).}
We randomly sample inputs with shape $(m, k, k, 3)$ where $m\in \{12, 20\}$ and $k=6$. We compute the exact NTK with activation function {\it Erf} using the {\it Neural Tangents} library~\citep{neuraltangents2019}. We see excellent agreement between the theoretical calculation of $\kappal$ in Sec.~\ref{sec:theory} (summarized in Table~\ref{table evolution ntk}) and the experimental results Figure~\ref{fig: conditioning-complete}.


\begin{figure*}[h]
\begin{center} 
\includegraphics[width=.93\textwidth]{new_graphs/graphs-test/heat-map-letter-horizontal-v25-2.pdf}
\end{center}
\caption{{\bf Trainability and generalization are captured by $\kappal$ and $\Deltal$.}
(a,b) The training and test accuracy of CNN-F trained with SGD. The network is untrainable above the green line because $\kappal$ is too large and is ungeneralizable above the orange line because $\Deltal$ is too small. (c) The accuracy vs learning rate for FCNs trained with SGD sweeping over the weight variance. (d,e) The test accuracy of CNN-P and CNN-F using kernel regression. (f) The difference in accuracy between CNN-P and CNN-F networks.}\label{fig:pool vs flatten}
\end{figure*}



{\bf Maximum Learning Rates (Figure~\ref{fig:pool vs flatten} (c)).} 
In practice, given a set of hyper-parameters of a network, knowing the range of feasible learning rates is extremely valuable. As discussed above, in the infinite width setting, \eqref{eq:fc_ntk_recap_dynamics} implies the maximal convergent learning rate is given by $\eta_{\rm theory} \equiv 2/ {\lambda^{(l)}_{\rm max}}$. From our theoretical results above, varying the hyperparameters of our network allows us to vary $\lambda^{(l)}_{\rm max}$ over a wide range and test this hypothesis. This is shown for depth 10 networks varying $\sigma_w^2$ with $\eta = \rho\eta_{\rm theory}$. We see that networks become untrainable when $\rho$ exceeds 2 as predicted. 

{\bf Trainability vs Generalization (Figure~\ref{fig:pool vs flatten} (a,b)).}
We conduct an experiment training finite-width CNN-F networks with 1k training samples from CIFAR-10 with $20\times 20$ different $(\sws, l)$ configurations. We train each network using SGD with batch size $b=256$ and learning rate $\eta = 0.1 \eta_{\rm theory}$. We see in Figure~\ref{fig:pool vs flatten} (a) that deep in the chaotic phase we see that all configurations reach perfect training accuracy, but the network completely fails to generalize in the sense test accuracy is around $10\%$. 
As expected, in the ordered phase we see that although the training accuracy degrades generalization improves. As expected we see that the depth-scales $\xi_1$ and $\xi_*$ control trainability in the ordered phase and generalization in the chaotic phase respectively. We also conduct extra experiments for FCN with more training points (16k); see Figure~\ref{fig:train-test-acc-fcn}. 

{\bf CNN-P v.s. CNN-F: spatial correction (Figure~\ref{fig:pool vs flatten} (d-f)).}
We compute the test accuracy using the analytic equations for gradient flow, \eqref{eq:ntk-predictor}, which corresponds to the test accuracy of ensemble of gradient descent trained neural networks taking the width to infinity.
As above, we use $1k$ training points and consider a $20\times 20$ grid of configurations for $(\sws, l)$. We plot the test performance of CNN-P and CNN-F and the performance difference in Fig \ref{fig:pool vs flatten} (d-f). As expected, we see that the performance of both CNN-P and CNN-F are captured by $\xi_1 = - 1/\log(\chi_1)$ in the ordered phase and by $\xi_* = -1/ (\log \xi_c - \log\xi_1)$ in the chaotic phase. We see that the test performance difference between CNN-P and CNN-F exhibits a region in the ordered phase (a blue strip) where CNN-F outperforms CNN-P by a large margin. This performance difference is due to the correction term $d$ as predicted by the $\Deltal$-row of Table~\ref{table evolution ntk}. We also conduct extra experiments densely varying $\sbs$; see Sec.~\ref{sec:varying-sb}. Together these results provide an extremely stringent test of 
our theory. 





